Design of Stochastic Robotic Swarms for Target Performance Metrics in Boundary Coverage Tasks

In this work, we analyze \textit{stochastic coverage schemes} (SCS) for robotic swarms in which the robots randomly attach to a one-dimensional boundary of interest using local communication and sensing, without relying on global position information or a map of the environment. Robotic swarms may be required to perform boundary coverage in a variety of applications, including environmental monitoring, collective transport, disaster response, and nanomedicine. We present a novel analytical approach to computing and designing the statistical properties of the communication and sensing networks that are formed by random robot configurations on a boundary. We are particularly interested in the event that a robot configuration forms a connected communication network or maintains continuous sensor coverage of the boundary. Using tools from order statistics, random geometric graphs, and computational geometry, we derive formulas for properties of the random graphs generated by robots that are independently and identically distributed along a boundary. We also develop order-of-magnitude estimates of these properties based on Poisson approximations and threshold functions. For cases where the SCS generates a uniform distribution of robots along the boundary, we apply our analytical results to develop a procedure for computing the robot population size, diameter, sensing range, or communication range that yields a random communication network or sensor network with desired properties.

==> Motiv.tex <==
\section{Motivation}
\label{Sec:Motiv} 
Suppose a team of robots is placed at random positions in a bounded environment. Robots are provided only with their (perfect) odometric readings and Wifi measurements, and a camera for detecting landmarks. Each robot is a disk of diameter $\dia$, and its Wi-fi has a communication radius of $\sat$. Likewise, it can sense and identify other objects within a sensing range of $\sat$. We take the robots' communication and sensing radii to be equal to each other $\sat$ only for computational convenience.    Robots have no knowledge of their global positions; nor are they provided with offboard sensing that helps them localize. Since the main thrust of this paper lies in the randomized analysis of the network created by the robots, we will make the following simplifying assumptions:  All robots are synchronized in time with respect to a global clock, and the robot controllers do not fail in the course of execution.  

In the environment is placed a line segment boundary $\Bo$, whose endpoints $\mathcal{B}_w$ and $\mathcal{B}_b$ are colored black and white respectively, distinctively from the rest of the environment. These colors can be identified by cameras mounted on each robot. We call any algorithm that results in the team claiming  positions on $\Bo$ a \textit{coverage scheme}.  Usually, we require that robot configurations on $\Bo$ to be \textit{conflict-free (CS)}, i.e. no robots physically overlaps with another, and \textit{conflict-tolerant (CT)}. We call the respective coverage schemes conflict-free and conflict tolerant. 

When the robot team claims (disjoint)  positions on the boundary in such a way that every robot is able to communicate with every other, we say that they form a \textit{connected} network; otherwise, they form a \textit{disconnected} network. Note that a robot team forms a connected network senses iff a (contiguous) subinterval of $\Bo$. Define the \textit{sensed subset} of $\Bo$ to be the set of points sensed by at least one robot. We say that $\Bo$ is \textit{fully sensed}, iff every point in it is sensed. Any configuration of multiple robots that fully senses $\Bo$ has to form a connected network. Finally, we say that a robot configuration on $\Bo$ \textit{monitors} $\Bo$ iff it is connected \textit{and} senses the entirety of $\Bo$.  


\input{Figs/Att1}

We will focus on \textit{stochastic coverage schemes(SCS)} in which the robot team chooses positions randomly on $\Bo$, and refer only briefly to their deterministic counterparts (DCS).  Our aim in this paper will be to analyze the communication network  generated by SCS, and to design the parameters $\dia$ and $\nor$ so that they generate a network with a guarantee on the probability $\pcon$ that it will fully sense $\Bo$. We motivate our work with the following problem scenarios:

\subsection{SCS for robots lacking odometry}
\label{Subsec:nodom}
In \cite{PavlicISRR2013, PavlicJSDSC14,WilsonSwarmInt2014}, we devised a stochastic controller for allocating a robot team to multiple boundaries, with the goal of achieving a target allocation on each boundary. The robots thus allotted to boundaries lacked the ability to localize, and had no odometry. They were instead programmed to do a \textit{correlated random walk} (CRW) in the environment, and followed a \textit{chemical reaction network} (CRN) to either attach or detach from a boundary that they sensed. We proved in  \cite{PavlicISRR2013} that our stochastic controller achieved its target allocation with a certain probability; however, we had little idea of the spatial distributions generated by the robot team attaching to a single boundary.  Nonetheless, we realized that if robots were uniformly distributed around an empty load boundary $\Bo$, each point on $\Bo$ was equally likely to be picked for attachment by the next attaching robot. On the other hand, a nonuniform spatial distribution is generated by a robot CRW with parameters resulting in a nonuniform spatial concentration of robots.  



\subsection{DCS for robots with noisy odometry}
\label{Subsec:dcsodom}
Consider coverage scheme in which robots position themselves one at a time on the boundary one at a time, spacing themselves $\sat$ apart, with $\Rob_{i}$ claiming equidistant positions (say  $\sat,2\sat,\ldots,$) from $\Bo_W$, until $\Bo$ is fully sensed.  This scheme ensures connectivity with complete certainty if wheel odometry is noise-free. However, in the presence of odometric noise, $\Rob_{i}$ will have a truncated Gaussian pdf with its mean located at $\upos{i}$. We call the resulting scheme a deterministic coverage  scheme (DCS) with noise. Suppose we are now given the variance $\sigma^2_i$ of each Gaussian pdf, and the values $\sat$ and $\nor$. We now ask the probability $\pcon$ with which $\G$ will be connected. 

It is clear that computing $\pcon$ involves computing the volume of a multivariate Gaussian defined by robot positions. However, it is unclear as to how well this computation of $\pcon$ generalizes to a situation in which (a) robot positions are correlated with each other (b) robots' odometry has a non-Gaussian noise profile (c) robots have distinct communication ranges. Further, \textit{design problems} such as computing the number of robots which will give us a connected network with say $95\%$ probability is quite a cumbersome task. 

\subsection {SCS for robots with perfect odometry}
\label{Subsec:scsodom}
There are other problem scenarios for which a stochastic coverage scheme (SCS) is preferable to a DCS. Suppose the robot team needs to collectively lift a heavy load \cite{KumarSHS2013,PavlicISRR2013} of whose mass distribution it has no prior knowledge. Then a good strategy to lift the load  involves placing robots randomly around the load boundary, lifting the load collectively. The clustering process continues until the load gets displaced, or until the robot team decides to give up. Alternatively, the team may recruit sufficiently many new members to be able to lift the load in unison. 

We are now confronted with the same problems as in \autoref{Subsec:dcsodom}, except that they involve the spatial distribution of attachment, instead of odometric noise profiles. For example, $\Rob_{1}$ attaches uniformly randomly to $\Bo$, and $\Rob_{2}$ attaches with a Gaussian pdf centered at $\Rob_{1}$. Next, $\Rob_{3}$ positions itself ``far away'' from $\Rob_{1}$ and $\Rob_{2}$, using a suitable spatial pdf. Computing the probability $\pcon$ is nontrivial, as is the variant in which robots have distinct communication ranges. 

Note the following important difference between SCS that are odometry-aided vs those that lack it. In the former case (as in \autoref{Subsec:dcsodom} and \autoref{Subsec:scsodom}), a sample of $\nor$ robots attaching randomly using the SCS is straightforward to draw by having the first robot attach independently, and subsquently having dependent robots taking up positions  conditioned on that of $\Rob_{1}$. If robot positions are independent and each position can be sampled in constant time, then an attachment of $\nor$ robots takes $O(n)$ time to sample. On the other hand, when the SCS lacks odometry, the robot population on a boundary rises and falls over time. Since the CRN rates are the only control we have on attachment, a configuration of $\nor$ robots takes longer to sample in general. While the network generated by either SCS has the same properties, the presence of a perfect odometer makes it possible for robots to actively coordinate to attach, in a way that was not possible with CRNs.  

This work will analyze  communication networks arising from a large class of SCS, thereby solving many (but not all) of the problems raised in \autoref{Subsec:nodom} through \autoref{Subsec:scsodom}. 









==> Results.tex <==
\section{Designing for Specific Graph Properties}
\label{Sec:results}

\subsection{Uniform Parents}



\subsection{General iid Parents}





  



==> Tabs/Tabcov1.tex <==
\begin{table}[t] %htbp
\caption{Estimating Position Covariance Matrices} 
\label{tab:poscov}
\centering
\begin{tabular}{ccc} 

\toprule
 & $\sla = 1 ~~ \nor = 3 ~~\rad = 0$ \\
\hline
$\Covm{\rvposvec}=$& $  \begin{matrix}
         0.037 &   0.025 &   0.0125 \\
         0.025  &  0.050  &  0.0250 \\
         0.012   & 0.025   & 0.037 \\
 \end{matrix} $ \\
 \noalign{\vskip 2mm}    
$\ECovm{\rvposvec}=$ &    $\begin{matrix}  
      0.037  &  0.025  &  0.013 \\
       0.025 &   0.050  &  0.025 \\
       0.012  &  0.026   & 0.038 \\
         \end{matrix}$\\
\bottomrule
         \end{tabular}

\end{table}


\begin{table}[t]
\caption{Estimating Slack Covariance Matrices} 
\label{tab:slackcov}
\centering
\begin{tabular}{ccc} 

\toprule
 & $\sla = 1 ~~ \nor = 3 ~~\rad = 0$ \\
\hline
$\Covm{\rvsvec}=$& $  \begin{matrix}
         0.037 &	-0.012 &	-0.012 &	-0.012 \\ 
 -0.013 &	0.037 &	-0.012 &	-0.012 \\ 
 -0.013 &	-0.012 &	0.037 &	-0.012 \\ 
 -0.013 &	-0.012 &	-0.012 &	0.038 \\ 
 \end{matrix} $ \\
 \noalign{\vskip 2mm}    
$\ECovm{\rvsvec}=$ &    $\begin{matrix} 
 0.037 &	-0.012 &	-0.013 &	-0.012\\ 
 -0.012 &	0.037 &	-0.013 &	-0.012 \\ 
 -0.013 &	-0.013 &	0.038 &	-0.013 \\ 
 -0.012 &	-0.012 &	-0.013 &	0.037 \\ 
         \end{matrix}$\\
\bottomrule
         \end{tabular}

\end{table}


==> Tabs/Tabequiv.tex <==
\begin{table}[t]
\centering
\caption{ Equivalence of Sampling Algorithms - 1 }%  
\vspace{-2mm}
\begin{tabular} {ll} % Put two tables side by side

\begin{tabular}{cccc}
\toprule
$\sla=1$ & $\rad=0$ & $\nor=2$ & $\sat = 0.6$ \\ 
Moment of $\rvsla{1}$  & REJSAMP &  GEOMSAMP &  REPSAMP \\ \hline  
$\Exp{\rvsla{1}}$ & 0.3317  &  0.3306 & 0.3317  \\ 
 
$\mu_2(\rvsla{1})$& 0.0246 & 0.0249 & 0.0248 \\
  
$\mu_3(\rvsla{1})$& 0.0000 & 0.0000 & 0.0000 \\
  
$\mu_4(\rvsla{1})$ & 0.0012 & 0.0012 & 0.0012 \\
  

 \bottomrule 
 \end{tabular}
 
 \end{tabular}
  \label{tab:equiv1}
  \end{table}
 
\begin{table}[t] %!htbp
 \centering
\caption{ Equivalence of Sampling Algorithms - 2 }%  
\vspace{-2mm}
\begin{tabular} {ll} % Put two tables side by side

\begin{tabular}{cccc}
\toprule
$\sla=1$ & $\rad=0$ & $\nor=5$ & $\sat = 0.6$ \\ 
Moment of $\rvsla{1}$ & REJSAMP &  GEOMSAMP &  REPSAMP \\ \hline  
$\Exp{\rvsla{1}}$ & 0.1996  &  0.1996 & 0.1996  \\ 
 
$\mu_2(\rvsla{1})$& 0.0211 & 0.0212 & 0.0214 \\
  
$\mu_3(\rvsla{1})$& 0.0021 & 0.0021 & 0.0021 \\
  
$\mu_4(\rvsla{1})$ & 0.0012 & 0.0012 & 0.0012 \\
  

 \bottomrule 
 \end{tabular}
 
 \end{tabular}
  \label{tab:equiv2}
  \end{table}
  
 


==> Tabs/Tablarge.tex <==
\begin{table}[!htbp]
\caption{ Pyramids for large $\sat$  }%  
\vspace{-2mm}
\begin{tabular} {ll} % Put two tables side by side
% sv1 =     0.4000         0    0.6000
 % sv2 =   0.6000         0    0.4000
% sv3 =  0.6000    0.4000         0
% sv4 =     0.4000    0.6000         0
% sv5 =   0    0.6000    0.4000
% sv6 =          0    0.4000    0.6000


\begin{tabular}{cccc}
\toprule 
$\sla=1$ & $\nor=2$ & $\sat = 0.6$\\

\hline
Figure  & Volume  & Copies     \\ \hline  
$\Pyr{1}$ & 0.0577 & 3   \\ 
 
$\Pyr{2}$&   0.0924 & 3 \\
 
 
\vspace {1mm}
$\favn$ & 0.4503 \\
$\ssimpn$ & 0.8660 \\
 \hline
 & $\Vol(\favn) / \Vol(\ssimpn) $ & 0.5200 \\

 & ${\psat}$ & 0.5200 \\
\bottomrule
 \end{tabular}
 
 \end{tabular}
  \label{tab:larged1}
  \end{table}

==> Tabs/Tabmarg.tex <==
  \begin{table}[t]
  \centering
\caption{ Point Robots: estimating $\rvposvec$ and $\rvsvec$ }%  
\vspace{-2mm}
\begin{tabular} {ll} % Put two tables side by side
\begin{tabular}{c p{1mm} p{1mm} cc}
\hline 
 $\sla=1$ & & & $\nor=4$ & $\rad = 0 $ \\ 
Variable &$a$ &  $b$ &  $\esta$ & $\estb$  \\ \hline  
$\rvsla{1},\rvpos{1}$ &1 &4 &  0.999 &   3.987   \\    
$\rvpos{2}$ & 2 & 3 &  2.004  & 2.991 \\
$\rvpos{3}$ & 3 & 2 &  
    2.958 &   1.960 \\
$\rvpos{4}$ & 4 & 1 & 
    4.010 & 1.002 \\   
 \hline 
 \end{tabular}
 \end{tabular}
  \label{tab:margpoint}
  \end{table}
 
 \begin{table}[t]
\caption{ Finite Robots: estimating $\rvshposvec$ and $\rvfsvec$ }%  
\vspace{-2mm}
\centering
\begin{tabular} {ll} % Put two tables side by side
\begin{tabular}{c p{1mm} p{1mm} c c}
\hline 
 $\sla=1$ & &  &$\nor=2$ & $\dia=0.04$ \\ 
Variable &$a$ &  $b$ &  $\esta$ & $\estb$  \\ \hline  
$\rvfsi{1},\rvshpos{1}$ &1 &2  &  1.026 & 2.047   \\    
$\rvfsi{2}$ & 1 & 2 & 1.055 & 2.089 \\
$\rvfsi{3}$ & 1 & 2 &  0.989 &   1.997 \\
$\rvshpos{2}$ & 2 &1 & 1.997 & 0.989 \\   
 \hline 
 \end{tabular}
 \end{tabular}
  \label{tab:margfin}
  \end{table}
 

==> Tabs/Tabpsat.tex <==
\begin{table}[t] % !htbp
\centering
\caption{ Point Robots: $\psat$ vs. $\epsat$  \cite{icraboundarycover} }%  
\vspace{-2mm}
\begin{tabular} {ll} % Put two tables side by side
\begin{tabular}{ccc}
\toprule
 $\sla=1$ & $\nor=16$ & $\rad =0$ \\ 
 $\sat$ &  $\psat$ &  $\epsat$ \\ \hline  
 0.05  &  0.0000 & 0.0000  \\ 
 
 0.10 & 0.0001 & 0.0001 \\
  
 0.20 & 0.4929 & 0.4925 \\
  
 0.25 & 0.7898 & 0.7913 \\
  
 0.33 & 0.9635 & 0.9651 \\
  
 0.50 & 0.9995 & 0.9997 \\
 \hline 
 \end{tabular}
 &
 \begin{tabular}{ccc}
\toprule  
  $\sla=1$ & $\sat=0.5$ & $\rad =0$ \\ 
 $\nor $ & $\psat$  & $\epsat$ \\  \hline 
 3 &  0.2500 & 0.2467  \\
 
 4 & 0.5000 & 0.5029 \\
  
 5 & 0.6875 & 0.6885 \\
  
 6  & 0.8125 & 0.8124 \\
  
 7 & 0.8906 & 0.8899 \\
   8 & 0.9375 & 0.9383 \\
\hline 
 \end{tabular}
 \end{tabular}
  \label{tab:psatpoint}
  \end{table}
 
 

 
 
  
  
  

==> Tabs/Tabsmall.tex <==
  \begin{table}[!htbp]
  
  \centering
\caption{ Estimating  $\rvsvec|\Sat$ and $\rvposvec|\Sat$ for small $\nor$}%  
\label{tab:smalld1}
\vspace{-2mm}
\begin{tabular} {ll} % Put two tables side by side
\begin{tabular}{c p{1mm} p{1mm} cc}
\hline 
 $\sla=1$ & $\rad=$ & 0 & $\nor=3$ & $\sat = 0.3 $ \\ 
 Variable &$a$ &  $b$ &  $\estb$ & $\esta$  \\ \hline  
$\rvsla{1},\rvpos{1} | \Sat$ &3 &1 &  2.860&   0.991   \\    
$\rvpos{2}|\Sat$ & 2 & 2 &  1.969 &   1.982 \\
$\rvpos{3}|\Sat$ & 1 & 3 & 0.986 & 2.826 \\   
 \hline 
 \end{tabular}
 \end{tabular}
\end{table}

\begin{table}[!htbp]
\caption{Estimating Slack Covariance Matrices for small $\nor$} 
\label{tab:smalld2}
\centering
\begin{tabular}{ccc} 

\toprule
 & $\sla = 1 ~~ \rad = 0 ~~ \nor = 3 ~~\sat = 0.3$ \\
\hline
$\Covm{\rvsvec|\Sat}=$& $  \begin{matrix}
   0.0015 &	-0.0005 &	-0.0005 &	-0.0005 \\ 
 -0.0005 &	0.0015 &	-0.0005 &	-0.0005 \\ 
 -0.0005 &	-0.0005 &	0.0015 &	-0.0005 \\ 
 -0.0005 &	-0.0005 &	-0.0005 &	0.0015 \\ 
 \end{matrix} $ \\
 \noalign{\vskip 2mm}    
$\ECovm{\rvsvec|\Sat}=$ &    $\begin{matrix} 
0.0015 &	-0.0005 &	-0.0005 &	-0.0005 \\ 
 -0.0005 &	0.0015 &	-0.0005 &	-0.0005 \\ 
 -0.0005 &	-0.0005 &	0.0015 &	-0.0005 \\ 
 -0.0005 &	-0.0005 &	-0.0005 &	0.0015 \\ 
         \end{matrix}$\\
\bottomrule
         \end{tabular}

\end{table}
